A Multi-Dataset Evaluation of Models for Automated Vulnerability Repair

Software vulnerabilities pose significant security threats, requiring effective mitigation. While Automated Program Repair (APR) has advanced in fixing general bugs, vulnerability patching, a security-critical aspect of APR remains underexplored. This study investigates pre-trained language models, CodeBERT and CodeT5, for automated vulnerability patching across six datasets and four languages. We evaluate their accuracy and generalization to unknown vulnerabilities. Results show that while both models face challenges with fragmented or sparse context, CodeBERT performs comparatively better in such scenarios, whereas CodeT5 excels in capturing complex vulnerability patterns. CodeT5 also demonstrates superior scalability. Furthermore, we test fine-tuned models on both in-distribution (trained) and out-of-distribution (unseen) datasets. While fine-tuning improves in-distribution performance, models struggle to generalize to unseen data, highlighting challenges in robust vulnerability detection. This study benchmarks model performance, identifies limitations in generalization, and provides actionable insights to advance automated vulnerability patching for real-world security applications.

==> tables/RQ2_results_CodeBERT.tex <==
\pgfplotstabletypeset[
    col sep=comma,
    empty cells with={-},
    every head row/.style={
        before row={\toprule},
        after row=\midrule,
    },
    every last row/.style={after row=\bottomrule},
    columns={Model,TrainedOn,TestedOn,CodeBLEU,CrystalBLEU},
    columns/Model/.style={
        column type=l, % Left-align
        string type, % Treat as strings
        column name={Model}, % Column header
    },
    columns/TrainedOn/.style={
        column type=l, 
        string type, 
        column name={Trained On}, 
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        }
    },
    columns/TestedOn/.style={
        column type=l, 
        string type, 
        column name={Tested On}, 
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        }
    },
    columns/CodeBLEU/.style={
        column type=r, 
        column name={CodeBLEU}, 
        precision=4, 
        fixed  % Ensure fixed-point notation
    },
    columns/CrystalBLEU/.style={
        column type=r, 
        column name={CrystalBLEU}, 
        precision=4, 
        fixed  % Ensure fixed-point notation
    },
    every row/.style={after row=\midrule}, % Midrule after each row
    % Highlighting rows
    highlight row/.style={
        before row={\rowcolor{gray!45}}, % Highlight row with gray
    },
    % Highlight every 6th row
    every nth row={6}{highlight row},  
    % Highlight the first row explicitly
    every first row/.style={highlight row}, 
]{data/RQ2_ease_Codebert.csv}


==> tables/RQ2_results_CodeT5.tex <==
\pgfplotstabletypeset[
    col sep=comma,
    empty cells with={-},
    every head row/.style={
        before row={\toprule},
        after row=\midrule,
    },
    every last row/.style={after row=\bottomrule},
    columns={Model,TrainedOn,TestedOn,CodeBLEU,CrystalBLEU},
    columns/Model/.style={
        column type=l, % Left-align
        string type, % Treat as strings
        column name={Model}, % Column header
    },
    columns/TrainedOn/.style={
        column type=l, 
        string type, 
        column name={Trained On}, 
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        }
    },
    columns/TestedOn/.style={
        column type=l, 
        string type, 
        column name={Tested On}, 
        postproc cell content/.code={%
            \pgfplotsutilstrreplace{_}{\_}{##1}%
            \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
        }
    },
    columns/CodeBLEU/.style={
        column type=r, 
        column name={CodeBLEU}, 
        precision=4, 
        fixed  % Ensure fixed-point notation
    },
    columns/CrystalBLEU/.style={
        column type=r, 
        column name={CrystalBLEU}, 
        precision=4, 
        fixed  % Ensure fixed-point notation
    },
    every row/.style={after row=\midrule}, % Midrule after each row
    % Highlighting rows
    highlight row/.style={
        before row={\rowcolor{gray!45}}, % Highlight row with gray
    },
    % Highlight every 6th row
    every nth row={6}{highlight row},  
    % Highlight the first row explicitly
    every first row/.style={highlight row}, 
]{data/RQ2_ease_Codet5.csv}


==> tables/RQ2_results_efficiency.tex <==
\pgfplotstabletypeset[
    col sep=comma,
    fixed,
    empty cells with={-},
    string replace={---}{\textemdash},
    string replace={_}{\textunderscore},
    every head row/.style={
        before row={\toprule},
        after row=\midrule,
    },
    every last row/.style={after row=\bottomrule},
    columns={Dataset,AvgInferenceTimeBERT,AvgInferenceTimeT5,testInstancesBERT}, 
    columns/Dataset/.style={column type=l, string type, postproc cell content/.code={%
        \pgfplotsutilstrreplace{_}{\_}{##1}%
        \pgfkeyslet{/pgfplots/table/@cell content}\pgfplotsretval
    }},
    columns/AvgInferenceTimeBERT/.style={column type=r,column name=$CodeBERT$, precision=4},
    columns/AvgInferenceTimeT5/.style={column type=r, column name=$CodeT5$, precision=4},
    columns/testInstancesBERT/.style={column type=r,column name=$Test Instances$, precision=4},
]{data/summary_RQ1_RQ2_ease_paper.csv}
